On the Construction of Quantum Field Theories with Factorizing S-Matrices

The subject of this thesis is a novel construction method for interacting relativistic quantum field theories on two-dimensional Minkowski space. The input in this construction is not a classical Lagrangian, but rather a prescribed factorizing S-matrix, i.e. the inverse scattering problem for such quantum field theories is studied. For a large class of factorizing S-matrices, certain associated quantum fields, which are localized in wedge-shaped regions of Minkowski space, are constructed explicitely. With the help of these fields, the local observable content of the corresponding model is defined and analyzed by employing methods from the algebraic framework of quantum field theory. The abstract problem in this analysis amounts to the question under which conditions an algebra of wedge-localized observables can be used to generate a net of local observable algebras with the right physical properties. The answer given here uses the so-called modular nuclearity condition, which is shown to imply the existence of local observables and the Reeh-Schlieder property. In the analysis of the concrete models, this condition is proven for a large family of S-matrices, including the scattering operators of the Sinh-Gordon model and the scaling Ising model as special examples. The so constructed models are then investigated with respect to their scattering properties. They are shown to solve the inverse scattering problem for the considered S-matrices, and a proof of asymptotic completeness is given.

==> PhD-bibliography.tex <==
\addcontentsline{toc}{chapter}{Bibliography}
\begin{thebibliography}{99}
\bibitem{AFZ} A.E.~Arinshtein, V.A.~Fateev, A.B.~Zamolodchikov, Quantum
  S-matrix of the $(1+1)$-dimensional Toda chain, {\it Phys. Lett.} {\bf B 87}
  (1979), 389-392.
 
\bibitem{KaBa} H.~Babujian, M.~Karowski, Exact form factors for the scaling $Z_N$-Ising
and the affine $A_{N-1}$-Toda quantum field theories, {\it Phys.Lett.}
{\bf B575} (2003), 144-150, [arXiv: hep-th/0309018].

\bibitem{BiWi} J.~J.~Bisognano, E.~H.~Wichmann, On the duality condition
  for a hermitian scalar field, {\it J. Math. Phys.} {\bf 16} (1975),
  985-1007, On the duality condition for quantum fields, {\it
    J. Math. Phys.} {\bf 17} (1976), 303-321.

\bibitem{boas} R.~P.~Boas, {\it Entire Functions}, Academic Press, New
  York, 1954.

\bibitem{bochner-martin} S.~Bochner, W.~T.~Martin, {\it Several
    Complex Variables}, $4^{\rm th}$ Ed., Princeton University Press,
  Princeton, 1948.

\bibitem{borchers} H.-J.~Borchers, The CPT theorem in two-dimensional
    theories of local observables, {\it Commun. Math. Phys.} {\bf 143}
    (1992), 315-332.

\bibitem{revolution} H.-J.~Borchers, On Revolutionizing Quantum Field
  Theory with Tomita's Modular Theory, {\it J.~Math.~Phys.} {\bf 41}
  (2000), 3604-3673, [e-print available under http://www.lqp.uni-goe.de/lqp/papers/99/04/99042900.html].

\bibitem{BBS}  H.-J.~Borchers, D.~Buchholz, B.~Schroer,
  Polarization-Free Generators and the S-Matrix, {\it
    Commun. Math. Phys.} {\bf 219} (2001), 125-140, [arXiv:
  hep-th/0003243].

\bibitem{BGL} R.~Brunetti, D.~Guido, R.~Longo, Modular localization
  and Wigner particles, {\it Rev. Math. Phys.} {\bf 14} (2002), 759-786, [arXiv: math-ph/0203021].

\bibitem{nuclearmaps1} D.~Buchholz, C.~D'Antoni, R.~Longo, Nuclear
    Maps and Modular Structures I: General Properties, {\it
      Journ. Funct. Anal.} {\bf 88} (1990), 233-250.

\bibitem{nuclearmaps2} D.~Buchholz, C.~D'Antoni, R.~Longo, Nuclear
    Maps and Modular Structures II: Applications to Quantum Field Theory,
  {\it Commun. Math. Phys.} {\bf 129} (1990), 115-138.

\bibitem{BuJu2} D.~Buchholz, P.~Junglas, Local Properties of
    Equlibrium States and the Particle Spectrum in Quantum Field
    Theory, {\it Lett.~Math.~Phys.} {\bf 11} (1986), 51-58.

\bibitem{BuLe} D.~Buchholz, G.~Lechner, Modular Nuclearity and
    Localization, {\it Ann. H. Poincar\'e} {\bf 5} (2004), 1065-1080, [arXiv: math-ph/0402072].

\bibitem{BuWi} D.~Buchholz, E.~H.~Wichmann, Causal Independence
    and the Energy-Level Density of States in Local Quantum Field
    Theory, {\it Commun. Math. Phys.} {\bf 106} (1986), 321-344.

\bibitem{BuSuAdS} D.~Buchholz, S.J.~Summers, Stable quantum systems in
  anti-de Sitter space: Causality, independence and spectral
  properties, {\it J.Math.Phys.} {\bf 45} (2004), 4810-4831, [arXiv: math-ph/0407011].

\bibitem{BS-scatter} D.~Buchholz, S.J.~Summers, Scattering in
  Relativistic Quantum Field Theory: Fundamental Concepts and Tools,
  [arXiv: math-ph/0509047].

\bibitem{BS-1} D.~Buchholz, S.J.~Summers [arXiv: math-ph/0512060].

\bibitem{castro} O.A.~Castro-Alvaredo, A.~Fring, C.~Korff, Form
  factors of the homogeneous sine-Gordon models, {\it Phys. Lett.}
  {\bf B 484} (2000), 167-176, [arXiv: hep-th/0004089].

\bibitem{dopl} S.~Doplicher, R.~Longo, Standard and split
    inclusions of von Neumann algebras, {\it Invent. Math.} {\bf
      75} (1984), 493-536.

\bibitem{duren} P.~L.~Duren, {\it Theory of $H^p$ spaces}, Dover
  Publications, Inc., Mineola, New York, 2000.

\bibitem{eden} R.~J.~Eden, P.~V.~Landshoff, D.~I.~Olive,
  J.~C.~Polkinghorne, {\it The analytic S-matrix}, Cambridge
  University Press, Cambridge, 1966.

\bibitem{epstein-eotw} H.~Epstein, Generalization of the
    ``Edge-of-the-Wedge'' Theorem, {\it J. Math. Phys.} {\bf 1}
    (1960), 524-531.

\bibitem{epstein66} H.~Epstein, Some Analytic Properties of
    Scattering Amplitudes in Quantum Field Theory, in {\it Axiomatic
      Field Theory}, M.~Chretien, S.~Deser (eds.), Gordon \& Breach,
    New York, 1966.

\bibitem{fring} A.~Fring, G.~Mussardo, P.~Simonetti, Form Factors for
  Integrable Lagrangian Field Theories, the Sinh-Gordon Model, {it
    Nucl.Phys.} {\bf B 393} (1993), 413-441, [arXiv: hep-th/9211053].

\bibitem{garnett} J.~B.~Garnett, {\it Bounded Analytic Functions},
  Academic Press, New York, 1981.

\bibitem{haag} R.~Haag, {\it Local Quantum Physics}, $2^{\rm nd}
Ed.$, Springer, Berlin, 1996.

\bibitem{iago} D.~Iagolnitzer, {\it Scattering in Quantum Field
    Theories}, Princeton University Press, Princeton, 1993.

\bibitem{karo} M.~Karowksi, H.J.~Thun, T.T.~Truong, P.H.~Weisz, On the
  uniqueness of a purely elastic S-matrix in (1+1) dimensions, {\it
    Phys.~Lett.} {\bf 67 B} (1977), 321-322.

\bibitem{kosaki} H.~Kosaki, On the continuity of the map
    $\varphi\to|\varphi|$ from the predual of a $W^*$-algebra, {\it
      J. Funct. Anal.} {\bf 59} (1984), 123-131.

\bibitem{krantz} S.~G.~Krantz, {\it Function Theory of Several Complex
    Variables}, $2^{\rm nd}$ Ed., Wadsworth \& Brooks, Pacific Grove, 1992.

\bibitem{gl1} G.~Lechner, Polarization-Free Quantum Fields and
    Interaction, {\it Lett. Math. Phys.} {\bf 64} (2003), 137-154, [arXiv:hep-th/0303062].
\bibitem{GL-1} G.~Lechner, On the existence of local observables
    in theories with a factorizing S-matrix, {\it J.~Phys.~A} {\bf 38}
    (2005), 3045-3056, [arXiv: math-ph/0405062].

\bibitem{gl-bros} G.~Lechner, Towards the construction of quantum
    field theories from a factorizing S-matrix, {\it preprint} (2005), [arXiv: hep-th/0502184].

\bibitem{gl-future} G.~Lechner, work in progress.

\bibitem{LiMi} A.~Liguori, M.~Mintchev, Fock Representations of Quantum
      Fields with Generalized Statistics, {\it Commun. Math. Phys.}
      {\bf 169} (1995), 635-652, [arXiv: hep-th/9403039].

\bibitem{BCFT} R.~Longo, K.-H.~Rehren, Local fields in boundary
  conformal QFT, {\it Rev.~Math.~Phys.} {\bf 16} (2004), 909-960, [arXiv:
  math-ph/0405067].

\bibitem{martin} A.~Martin, Can one continue the scattering
    amplitude through the elastic cut?, in {\it Problems in
      Theoretical Physics}, D.~I.~Blokintseff (editor), Nauka, Moscow,
    1969, p. 113.

\bibitem{mitra} P.~Mitra, Elasticity, Factorization and
    S-Matrices in (1+1)-Dimensions, {\it Phys. Lett.} {\bf 72 B} (1977), 62-64.

\bibitem{mueger-w-split} M.~M\"uger, Superselection structure of
    massive quantum field theories in 1+1  dimensions,
  {\it Rev.~Math.~Phys.} {\bf 10} (1998), 1147-1170, [arXiv: hep-th/9705019].

\bibitem{simon-reed-2} M.~Reed, B.~Simon, {\it Methods of modern
    mathematical physics II: Fourier Analysis, Self-Adjointness},
  Academic Press, New York, 1975.

\bibitem{simon-reed-3} M.~Reed, B.~Simon, {\it Methods of modern
    mathematical physics III: Scattering Theory}, Academic Press, New
  York, 1979.

\bibitem{schroer} B.~Schroer, Modular wedge localization and the
  $d=1+1$ formfactor program, {\it Ann. Phys.} {\bf 275} (1999), 190-223, [arXiv: hep-th/9712124].

\bibitem{uniqueness} B.~Schroer, Uniqueness of Inverse Scattering
    Problem in Local Quantum Physics, {\it Ann. Phys.} {\bf 307}
    (2003), 421-437, [arXiv: hep-th/0106066].

\bibitem{schroer-wiesbrock}  B.~Schroer, H.-W.~Wiesbrock, Modular
  Constructions of Quantum Field Theories with Interactions, {\it Rev.~Math.~Phys.} {\bf 12} (2000), 301-326, [arXiv:hep-th/9812251].

\bibitem{smirnov} F.~A.~Smirnov, {\it Formfactors in completely
    integrable models in quantum field theory}, World Scientific,
  Singapore, (Advanced Series in Mathematical Physics vol. 14), 1992.

\bibitem{wiesbrock-2d} H.-W.~Wiesbrock, Symmetries and Half-Sided
  Modular Inclusions of von Neumann Algebras, {\it Lett.~Math.~Phys.} {\bf
  28} (1993), 107-114.

\bibitem{zamo} A.~Zamolodchikov, A.~Zamolodchikov, Factorized
    S-Matrices as the Exact Solutions of Certain Relativistic Quantum
    Field Theory Models, {\it Ann. Phys.} {\bf 120}  (1979), 253-291.

\end{thebibliography}

